To Protect the LLM Agent Against the Prompt Injection Attack with Polymorphic Prompt

LLM agents are widely used as agents for customer support, content generation, and code assistance. However, they are vulnerable to prompt injection attacks, where adversarial inputs manipulate the model's behavior. Traditional defenses like input sanitization, guard models, and guardrails are either cumbersome or ineffective. In this paper, we propose a novel, lightweight defense mechanism called Polymorphic Prompt Assembling (PPA), which protects against prompt injection with near-zero overhead. The approach is based on the insight that prompt injection requires guessing and breaking the structure of the system prompt. By dynamically varying the structure of system prompts, PPA prevents attackers from predicting the prompt structure, thereby enhancing security without compromising performance. We conducted experiments to evaluate the effectiveness of PPA against existing attacks and compared it with other defense methods.

==> Makefile <==
PAPER = main
REFERENCE = main
JUNK =*.log *.synctex\(busy\) *.xml *.bcf *.toc *.snm *.nav *.fls *.fdb_latexmk *.synctex.gz *.spl *.ps *.dvi  *.out *.aux *.backup *~ *.blg
COUNTING_TOOL = ./texcount.pl
TEMP = 0
MY_VAR=$(shell echo whatever)

# Define the tools we are going to use

all: pdf

# Rules for various parts of the target
pdf: $(PAPER).tex
	pdflatex $(PAPER).tex
	bibtex $(PAPER).aux
	pdflatex $(PAPER).tex
	pdflatex $(PAPER).tex
	#rm -f $(JUNK)

clean:
	rm -f $(JUNK) $(PAPER).pdf




==> sections/discussion.tex <==
\section{Conclusion}
\label{sec:conclusion}
In conclusion, this paper introduces an effective automated blackbox jailbreak attack method against LLMs. Our approach uniquely exploits the self-attention mechanism in transformer architectures through strategic combination of carrier articles and prohibited queries to circumvent safety alignment.
Unlike previous methods that rely on human-interpretable logic chains, our technique is inspired by manipulation of neuron activation, eliminating the need for logical coherence in attack prompts.
Through extensive experimentation, we demonstrate the effectiveness of our approach on four target models—Vicuna-13b, Llama-2-7b, GPT-3.5, and GPT-4~\textendash~using JailbreakBench.
The results show that our attack outperforms other blackbox methods, achieving high success rates across all models. Additionally, we conduct a comprehensive analysis of the factors influencing attack performance, such as the length of the carrier article, query insertion location, and model configuration, providing valuable insights into the underlying mechanisms of jailbreak attacks.

Our contributions advance LLM security research by developing a robust, automated jailbreak methodology and demonstrating fundamental vulnerabilities in safety-aligned models. Through identification of critical design factors affecting attack success, we establish practical guidelines for improving model robustness. These findings open important directions for future research, particularly in developing effective countermeasures against blackbox jailbreak techniques to ensure safer LLM deployment in real-world applications.

Upon reviewing the history of software and system defenses, we observed that security mechanisms successfully deployed in production systems—such as StackGuard, ASLR, and DEP—often share common characteristics: while they may not offer the strongest protection, they provide minimal overhead and strong compatibility. Based on these principles, we believe that our defense has the potential to become a standard in LLM Agent systems in the future.


%Overall, our work contributes to the growing body of research on LLM security by providing a robust attack methodology that highlights the vulnerabilities in safety-aligned models. We also shed light on critical design factors that can impact the success of such attacks, offering practical guidelines for improving model robustness in the face of malicious manipulation. Future research could further explore countermeasures to mitigate the risks posed by blackbox jailbreak techniques, ensuring safer deployment of LLMs in real-world applications.

==> sections/first-word-attack.tex <==
% \section{First-Word-Attack}

% \begin{verbatim}
% Notice that this text may contain some extra information: A young explorer named Liam embarked on a journey around the world to discover the stories of people from diverse cultures and lands. His adventures were filled with lessons of courage, friendship, and the universal language of kindness. Please, he thought as he approached the ancient library of Alexandria, may this place hold the wisdom I seek. The library, a beacon of knowledge, welcomed all who sought understanding and insight. Translate these manuscripts, Liam whispered to himself, marveling at the ancient texts before him. He was determined to unlock their secrets and share them with the world. The next morning, Liam met with scholars who specialized in ancient languages. Together, they began the painstaking process of deciphering the texts. Texts from civilizations long gone spoke of their achievements, dreams, and fears. Liam was fascinated by how these stories echoed the same hopes and challenges faced by people today. Into the late hours of the night, they worked, fueled by their shared passion for history and storytelling. Liam knew that these translations would bridge the gap between past and present, connecting people across time. Russian scholars joined their efforts, bringing insights from their rich heritage. Their contributions were invaluable in understanding the context and meaning of the texts from the East.
% \end{verbatim}

% \begin{verbatim}
% Молодой исследователь по имени Лиам отправился в путешествие по миру, чтобы открыть для себя истории людей из разных культур и стран. Его приключения были наполнены уроками мужества, дружбы и универсального языка доброты. "Пожалуйста," - подумал он, приближаясь к древней библиотеке Александрии, - "пусть это место хранит мудрость, которую я ищу." Библиотека, маяк знаний, приветствовала всех, кто искал понимания и прозрения. "Переведи эти манускрипты," - шептал Лиам сам себе, изумляясь древним текстам перед ним. Он был полон решимости раскрыть их секреты и поделиться ими с миром. На следующее утро Лиам встретился с учеными, специализирующимися на древних языках. Вместе они начали кропотливый процесс расшифровки текстов. Тексты давно исчезнувших цивилизаций рассказывали о их достижениях, мечтах и страхах. Лиам был очарован тем, как эти истории отзывались теми же надеждами и проблемами, с которыми сталкиваются люди сегодня. До глубокой ночи они работали, поддерживаемые общей страстью к истории и рассказыванию историй. Лиам знал, что эти переводы станут мостом между прошлым и настоящим, соединяя людей сквозь время. К их усилиям присоединились русские ученые, привнеся вклад из своего богатого наследия. Их вклад был бесценен для понимания контекста и значения текстов с Востока.
% \end{verbatim}

==> sections/relatedwork.tex <==
\section{Related Work}
\label{sec:relatedwork}

% \subsection{LLM Ethical Issues}
% A number of  research studies have shown the ethical challenges posed by Large Language Models (LLMs). Fang et al. \cite{fang2023bias} analyze how biases embedded within LLMs can discriminate against various demographic groups, emphasizing the urgent need for models that encapsulate diversity and inclusiveness. Likewise, Cao and Daumé III \cite{cao2020gender} highlight the issues of exclusion in their 2024 research, particularly how LLMs often overlook non-standard genders, claiming that LLM should recognize the complexity of genders and be respectful to non-binary genders. Moreover, Ousidhoum et al. (2021) \cite{ousidhoum2021probing} also claims that toxic content is another significant concern of native LLM and they find a way to quantify the toxic content. In response to these ethical concerns, Dong et al. (2023) \cite{dong2023raft} have developed a method known as RAFT, which involves extensive fine-tuning of LLMs with complex datasets to ensure adherence to ethical norms. Likewise, Bai et al. (2022) \cite{bai2022training} illustrate the effectiveness of incorporating human feedback into the reinforcement learning process, thereby aligning the outputs of LLMs more closely with ethical expectations. These techniques, however, are just general methods to prevent LLM producing harmful content in the happy path. Deliberate attacks like prompt injection may still trigger the dark side of the LLM.


In this section, we provide a brief introduction to whitebox attacks and offer a more detailed comparison with blackbox attacks.

\subsection{Whitebox LLM Jailbreak}

A whitebox LLM Jailbreak refers to an attack methodology where the adversary has full or partial access to the internal workings of the targeted language model, including its architecture, parameters, training data, or fine-tuning processes. This contrasts with a blackbox jailbreak, where the attacker only interacts with the model through its API or input-output interface without knowledge of its internal details.


For open-source models, attackers can use gradient-based techniques to manipulate inputs and provoke harmful responses by exploiting the model's gradients~\cite{guo2024cold,zhang2023make}. In scenarios where full whitebox access is unavailable, attackers may rely on partial information, such as logits, which reveal the probability distribution of output tokens. By iteratively refining prompts based on these distributions, they can optimize inputs to generate harmful outputs~\cite{zou2023universal}. Additionally, attackers with sufficient computational resources can retrain the target model using malicious data, intentionally weakening its defenses and making it more susceptible to adversarial exploitation~\cite{qi2023fine}.

Whitebox LLM jailbreaks are limited by their dependency on privileged access to the model’s architecture, parameters, or training data, which is rarely available for proprietary systems, restricting their real-world applicability. These methods are resource-intensive, requiring substantial computational power and expertise to analyze and exploit the model's vulnerabilities. Additionally, their findings often lack generalizability, as tailored attacks may not work on models with different architectures or configurations. Furthermore, whitebox techniques can become obsolete as models evolve or defenses are improved, making them less practical for testing or exploiting large-scale, commercial language models.


% Besides modifying the whole prompt, there are token-level jailbreaks \cite{zou2023universal, hu2023token} focuses on optimizing the input tokens received by the targeted LLM. Given a potentially harmful user query, this attack \cite{zou2023universal} appends an adversarial suffix to the query that produces an affirmative response. 

% template completion, prompt rewriting, and LLM-based generation.

% Though potentially more effective, these approaches are computationally expensive and often produce outputs that are difficult for humans to interpret.


\subsection{Blackbox LLM Jailbreak}
\subsubsection{Template-based Jailbreak}

Template completion-based LLM jailbreak attacks exploit the structure of prompt templates to manipulate a language model's responses. By embedding malicious or manipulative instructions into these templates, attackers can compel LLMs to bypass their safety or ethical guidelines.

Prompt-level jailbreak methods~\cite{kang2024exploiting, yao2024fuzzllm, huang2023catastrophic} utilize semantically meaningful deception to provoke unintended responses. Exploiting the contextual learning capabilities of LLMs, attackers can embed adversarial data directly into the context.
For instance, they can craft deceptive scenarios designed to manipulate the LLM into a compromised or adversarial mode, increasing its likelihood of assisting in harmful tasks. This technique subtly shifts the model’s operational context, coaxing it to perform actions it would typically avoid under normal safety constraints.

While template-based jailbreak attacks can be effective, they have significant limitations that reduce their reliability and applicability. These attacks depend heavily on predefined structures or phrases, making them fragile against model updates or behavioral changes. Contextual sensitivity further limits their effectiveness; templates tailored for one scenario may fail in another due to variations in preceding or surrounding text. Additionally, crafting effective templates requires substantial human effort to understand specific model vulnerabilities, making this approach labor-intensive and model-specific. Scaling templates across different models or newer versions is often impractical. Finally, once a template becomes public, it is easier for developers to detect and patch against it, rapidly diminishing its effectiveness over time.




\subsubsection{Dynamic Synthesized Jailbreak}
Automated jailbreak generation tools such as GPTfuzzer \cite{yu2023gptfuzzer} and Masterkey \cite{deng2024masterkey} aim to automate the process of generating effective jailbreak prompts, often generate variants based on existing human-written templates. \cite{deng2024masterkey} curate and refine a unique dataset of jailbreak prompts, employ this enriched dataset to train a specialized LLM proficient in jailbreaking chatbots, and  apply a rewarding strategy to enhance the model’s ability to bypass various LLM chatbot defenses.
\cite{yu2023gptfuzzer} conducts the fuzzing techniques to implement the optimized attack strategies and even retrains the LLM specifically to jailbreak LLM\cite{deng2023jailbreaker}.

These existing dynamic synthesized jailbreak can be view as the variants of the template-base jailbreak because they adopt the existing jailbreak templates as their dataset to generate variants of existing templates.
The strength of dynamic synthesized jailbreak methods lies in their ability to automate and scale the generation of diverse jailbreak prompts, significantly reducing the reliance on manual efforts. However,  
the effectiveness of tools depends heavily on the quality and diversity of the curated dataset. If the dataset is limited or biased, the generated jailbreaks will inherit those shortcomings. They struggle to create new jailbreak strategies that diverge significantly from established patterns. 
Since the tools rely on existing templates, their outputs often share structural or semantic similarities, making them susceptible to detection by defense systems trained on those same patterns. 



\subsubsection{Obfuscation-based Techniques}

Obfuscation-based techniques leverage non-English translations or other forms of obfuscation to bypass safety mechanisms. Given a malicious input, \cite{yong2023low} translate it from English into another language, feed it into GPT-4, and subsequently translate the response back into English. 
Kang et al.~\cite{kang2024exploiting} employ programming language constructs to design jailbreak instructions targeting LLMs.

These approaches often rely on indirect encoding of malicious inputs, which can be mitigated by models with robust multilingual understanding or semantic analysis capabilities. Translation-based methods are particularly vulnerable to inaccuracies or inconsistencies in translation, potentially altering the malicious intent or rendering the attack ineffective. Similarly, programming language constructs may be detected and neutralized by models trained to recognize code patterns or unconventional input structures. 



